Leveraging Spatial and Temporal Correlations in Sparsified Mean Estimation

We study the problem of estimating at a central server the mean of a set of vectors distributed across several nodes (one vector per node). When the vectors are high-dimensional, the communication cost of sending entire vectors may be prohibitive, and it may be imperative for them to use sparsification techniques. While most existing work on sparsified mean estimation is agnostic to the characteristics of the data vectors, in many practical applications such as federated learning, there may be spatial correlations (similarities in the vectors sent by different nodes) or temporal correlations (similarities in the data sent by a single node over different iterations of the algorithm) in the data vectors. We leverage these correlations by simply modifying the decoding method used by the server to estimate the mean. We provide an analysis of the resulting estimation error as well as experiments for PCA, K-Means and Logistic Regression, which show that our estimators consistently outperform more sophisticated and expensive sparsification methods.

==> Misc/Checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Proofs/randk_adap_proof.tex <==


Our goal is the following objective

\begin{align*}
\min_{w_1,w_2,\cdots,w_n} \frac{\frac{a_1}{w_1^2} + \frac{a_2}{w_2^2} + \cdots + \frac{a_n}{w_n^2}}{\left(\frac{b_1}{w_1} + \frac{b_2}{w_2} + \cdots + \frac{b_n}{w_n}\right)^2}
\end{align*}

Let $x_i = \frac{1}{w_i}$ and $\mathbf{x} = [x_1,x_2,\cdots,x_n]$. Let $\mathbf{b} = [b_1,b_2\cdots,b_n]$, $\mathbf{a} = [a_1,a_2\cdots,a_n]$ and $\mathbf{A} = diag(\mathbf{a})$. Our objective can alternately be written as,
\begin{align*}
    \min_{\mathbf{x}} \frac{\mathbf{x}^{T}\mathbf{A}\mathbf{x}}{(\mathbf{b}^{T}\mathbf{x})^2}
\end{align*}
Upon taking the derivative of above objective and setting it to 0, we get the following equation
\begin{align*}
    (\mathbf{x}^{T}\mathbf{b})\mathbf{A}\mathbf{x} - (\mathbf{x}^{T}\mathbf{A}\mathbf{x})\mathbf{b} = 0
\end{align*}
We observe that $\mathbf{x} = \mathbf{A}^{-1}\mathbf{b} = \frac{1}{\mathbf{a}} * \mathbf{b}$ is a solution of this equation.


Replacing our expressions for $a_m$ and $b_m$ as follows,
\begin{align*}
    a_m = \binom{n-1}{m-1}p^{m-1}(1-p)^{n-m} + p*\frac{S_2}{S_1}\binom{n-2}{m-2}p^{m-2}(1-p)^{n-m}
\end{align*}
\begin{align*}
    b_m = \binom{n-1}{m-1}p^{m-1}(1-p)^{n-m} 
\end{align*}
We get,
\begin{align*}
    w_i &= \frac{a_i}{b_i}\\
    & = 1 + \frac{S_2}{S_1}\frac{\binom{n-2}{i-2}}{\binom{n-1}{i-1}}\\
    & = 1 + \frac{S_2}{S_1}\frac{i-1}{n-1}
\end{align*}



\textbf{Reformulation of objective:}


Let $x_1 = 1$ and $\mathbf{y} = [\frac{x_1}{x_2},\cdots,\frac{x_1}{x_n}]$. Let $\mathbf{b} = [b_2\cdots,b_n]$, $\mathbf{a} = [a_2\cdots,a_n]$ and $\mathbf{A} = diag(\mathbf{a})$. Our objective can alternately be written as,
\begin{align*}
    \min_{\mathbf{y}} \frac{a_1 + \mathbf{y}^{T}\mathbf{A}\mathbf{y}}{(b_1 + \mathbf{b}^{T}\mathbf{y})^2}
\end{align*}
We also see that $a_1 = b_1$ in this case so we have,
\begin{align*}
    \min_{\mathbf{y}} \frac{a_1 + \mathbf{y}^{T}\mathbf{A}\mathbf{y}}{(a_1 + \mathbf{b}^{T}\mathbf{y})^2}
\end{align*}
Alternatively we also have,
\begin{align*}
    \min_{\mathbf{y}} \frac{a_1 + \mathbf{y}^{T}\mathbf{A}\mathbf{y}}{(a_1^2 + \mathbf{y}^{T}(\mathbf{b}\mathbf{b}^{T})\mathbf{y} + 2a_1\mathbf{b}^{T}\mathbf{y})}
\end{align*}


Taking the derivative as before and setting the numerator to 0 we have,
\begin{align*}
    & (a_1 + \mathbf{b}^{T}\mathbf{y})\left( (a_1 + \mathbf{b}^{T}\mathbf{y}) \mathbf{A}\mathbf{y} - (a_1 + \mathbf{y}^{T}\mathbf{A}\mathbf{y})\mathbf{b} \right) = 0 \\
    & = (a_1 + \mathbf{b}^{T}\mathbf{y})\left( a_1(\mathbf{A}\mathbf{y} - \mathbf{b}) + (\mathbf{b}^{T}\mathbf{y}) \mathbf{A}\mathbf{y} -  (\mathbf{y}^{T}\mathbf{A}\mathbf{y})\mathbf{b} \right)
\end{align*}


We can write the above inner expression as,
\begin{align*}
    \left( (\left(a_1 + \mathbf{b}^{T}\mathbf{y})\mathbf{I}- \mathbf{b}\mathbf{y}^{T}\right) (\mathbf{A}\mathbf{y}-\mathbf{b} \right))
\end{align*}

Can we show that $a_1 + \mathbf{b}^{T}\mathbf{y})\mathbf{I}- \mathbf{b}\mathbf{y}^{T} $ is full-rank?


We see that $\mathbf{y} = \mathbf{A}^{-1}\mathbf{b}$ is a solution of the above objective. 



Our objective can be written as,
\begin{align*}
    \min_{\y} f(\y) = \frac{a_1 + \y^{T}\A\y}{(a_1 + \b^{T}\y)^2}
\end{align*}

Taking the derivative of the objective we get,

\begin{align*}
    & \frac{((a_1 + \b^{T}\y)\mathbf{I}- \b\y^{T}) (\A\y-\b) }{(a_1+\b^T\y)^3}\\
    & = \frac{\H(\A\y-\b)}{(a_1+\b^T\y)^3}
\end{align*}
where $\H = (a_1 + \b^{T}\y)\mathbf{I}- \b\y^{T}$

\textbf{Proof to be shown:} $\H$ is full rank for $a_1 \neq \b^T\y$. 

Assuming the above holds true, for $\H(\A\y-\b) = 0$ we must have $\A\y-\b = 0 \implies \y = \A^{-1}\b$. 

Therefore the extrema points of our objective are given by $\A^{-1}\b$, $+\infty$, $-\infty$ and $-\b\frac{a_1}{\b^T\b}$. 

Assuming $a_1 > 0$ and $\A$ positive definite we can see that that $f(\y) \rightarrow \infty$ at $\y = -\b\frac{a_1}{\b^T\b}$. 

At $\y = \infty,-\infty$ we have, $f(\y) = \frac{sum(\A)}{sum(\b\b^T)}$. 

